Quantized Fourier and Polynomial Features for more Expressive Tensor Network Models

In the context of kernel machines, polynomial and Fourier features are commonly used to provide a nonlinear extension to linear models by mapping the data to a higher-dimensional space. Unless one considers the dual formulation of the learning problem, which renders exact large-scale learning unfeasible, the exponential increase of model parameters in the dimensionality of the data caused by their tensor-product structure prohibits to tackle high-dimensional problems. One of the possible approaches to circumvent this exponential scaling is to exploit the tensor structure present in the features by constraining the model weights to be an underparametrized tensor network. In this paper we quantize, i.e. further tensorize, polynomial and Fourier features. Based on this feature quantization we propose to quantize the associated model weights, yielding quantized models. We show that, for the same number of model parameters, the resulting quantized models have a higher bound on the VC-dimension as opposed to their non-quantized counterparts, at no additional computational cost while learning from identical features. We verify experimentally how this additional tensorization regularizes the learning problem by prioritizing the most salient features in the data and how it provides models with increased generalization capabilities. We finally benchmark our approach on large regression task, achieving state-of-the-art results on a laptop computer.

==> Fourier/large.tex <==
\begin{table*}[p]
\centering
\sisetup{table-align-uncertainty=true,
        retain-zero-uncertainty=true,
        separate-uncertainty=true,
        scientific-notation = false,
        table-alignment-mode=none}
\caption{Mean squared error (MSE) for different kernel machines on the airline dataset with one standard deviation. We report the number of basis functions $M$ per dimensions (in case of random approaches we simply report the total number of basis) and model parameters $P$. Keep in mind that the model parameters of QTKM (our approach) are complex-valued.
Notice that QTKM is able to parsimoniously predict airline delay with a restricted number of model parameters, achieving state-of-the art performance on this dataset.}
\robustify \bfseries
\label{tbl:large}
\begin{tabular}{
l
S[table-number-alignment = center]
S[table-number-alignment = center]
S[table-format=1.3(4),detect-weight]
}
\toprule                           
{Method}    &   {$M$}   &   {$P\downarrow$}   &   {MSE} \\
\cmidrule{1-4}
VFF \citep{hensman_variational_2017}              &   40    &  320   &   0.827 \pm 0.004 \\
Hilbert-GP \citep{solin_hilbert_2020}             &   40    &  320   &   0.827 \pm 0.005 \\
VISH \citep{dutordoir_sparse_2020}                &   660    &  660   &   0.834 \pm 0.055 \\
SVIGP \citep{hensman_gaussian_2013}               &   1000   &  1000  &   0.791 \pm 0.005 \\
T-KRR ($R=20$) \citep{wesel_large-scale_2021}     &   40     &  6400  &   0.763 \pm 0.007 \\       
Falkon \citep{meanti_kernel_2020}                 &   10000  &  10000 &   0.758 \pm 0.005 \\
\cmidrule{1-4}
QTKM ($R=20$)        &   64     &  1920  &   0.764 \pm 0.005 \\
% QTKM ($R=25$)        &   64     &  2400  &   0.757 \pm 0.005 \\
QTKM ($R=30$)        &   64     &  2880  &   0.754 \pm 0.005 \\
% QTKM ($R=35$)        &   64     &  3360  &   0.751 \pm 0.005 \\
QTKM ($R=40$)        &   64     &  3840  &  \bfseries 0.748 \pm 0.005 \\
\bottomrule
\end{tabular}
\end{table*}

==> Regularization.tex <==
\begin{figure*}
    %\captionsetup{font=normalsize,labelfont={bf,sf}}
    %\captionsetup[sub]{font=small,labelfont={bf,sf}}
    \centering
    \begin{subcaptionblock}[T][][c]{.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Regularization/yachtTest.pdf}
    \end{subcaptionblock}%
    \begin{subcaptionblock}[T][][c]{.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Regularization/qsarTest.pdf}
    \end{subcaptionblock}%
    \begin{subcaptionblock}[T][][c]{.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Regularization/energyTest.pdf}
    \end{subcaptionblock}%
    \begin{subcaptionblock}[T][][c]{.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Regularization/qsarfishTest.pdf}
    \end{subcaptionblock}\newline
    \begin{subcaptionblock}[T][][c]{.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Regularization/concreteTest.pdf}
    \end{subcaptionblock}%
    \begin{subcaptionblock}[T][][c]{.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Regularization/airfoilTest.pdf}
    \end{subcaptionblock}%
    \begin{subcaptionblock}[T][][c]{.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Regularization/wineTest.pdf}
    \end{subcaptionblock}%
    \begin{subcaptionblock}[T][][c]{.25\textwidth}
    \centering
    \includegraphics[width=\textwidth]{Regularization/bananaTest.pdf}
    \end{subcaptionblock}%
    \caption{Plots of the test mean squared error as a function of the number of model parameters $P$, for different real-life datasets. In blue, random Fourier features \citep{rahimi_random_2007}, in red tensorized kernel machines with Fourier features \citep{wahls_learning_2014,stoudenmire_supervised_2016,kargas_supervised_2021,wesel_large-scale_2021}, in yellow quantized kernel machines with Fourier features, with quantization $Q=2$. The gray horizontal full line is the full unconstrained optimization problem, which corresponds to kernel ridge regression (KRR). The grey vertical dotted line is set at $P=N$. It can be seen that in the underparametrized case, quantization allows to achieve better generalization performance with respect to the non-quantized case.} 
    \label{fig:generalization}
\end{figure*}

==> sound.tex <==
\begin{table}[h]
\centering
\sisetup{scientific-notation = false,
        table-number-alignment=center,
        table-alignment-mode=none}
\caption{Model parameters, compression ratio and relative approximation error of the weights, and standardized mean absolute error on the test data as a function of the CPD rank.}
\label{tbl:sound}
\begin{tabular}{
S[table-number-alignment = center]
S[table-number-alignment = center]
S[table-format=2.1]
S[table-format=1.3]
S[table-format=1.3]
}
\toprule                           
 {$R$}                &  {$P$}            & {$\nicefrac{M}{P}$}     & {$\nicefrac{\vert\vert\mat{w}-\mat{w}_\text{CPD}\vert\vert}{\vert\vert\mat{w}\vert\vert}$}    & {SMAE}             \\
\cmidrule{1-5}
10              & 260   &  31.5  &  0.841  &  0.579  \\
25              & 650   &  12.6  &  0.712  &  0.571  \\
50              & 1300  &  6.3  &  0.528  &  0.451   \\
100             & 2600  & 3.1   &  0.310  &  0.182   \\
\bottomrule
\end{tabular}
\end{table}
